Fast Kronecker Matrix-Matrix Multiplication on GPUs

Kronecker Matrix-Matrix Multiplication (Kron-Matmul) is the multiplication of a matrix with the Kronecker Product of several smaller matrices. Kron-Matmul is a core operation for many scientific and machine learning computations. State-of-the-art Kron-Matmul implementations utilize existing tensor algebra operations, such as matrix multiplication, transpose, and tensor matrix multiplication. However, this design choice prevents several Kron-Matmul specific optimizations, thus, leaving significant performance on the table. To address this issue, we present FastKron, an efficient technique for Kron-Matmul on single and multiple GPUs. FastKron is independent of linear algebra operations enabling several new optimizations for Kron-Matmul. Thus, it performs up to 40.7x and 7.85x faster than existing implementations on 1 and 16 GPUs respectively.

==> results/Makefile <==
all: small-singlegpu large-singlegpu large-8GPUs batch_size-8GPUs kernel_selection-small kernel_selection-large

small-singlegpu: small_batch_size_float_and_double.py
	python3 small_batch_size_float_and_double.py results-M\=16.csv results-M\=16-double.csv 4 64 $@.pdf ms False

# large-singlegpu-double: max_d.py
# 	python3 max_d_only_speedup.py results-M\=16.csv 4 64 $@.pdf ms False

# large-singlegpu: large-kron-4-16-yaxis.pdf large-kron-8-16.pdf large-kron-16-16.pdf large-kron-32-16.pdf

# large-kron-%-16-yaxis.pdf: singlegpu.py
# 	python3 singlegpu.py results-M\=320.csv $* 4 1

# large-kron-%-16.pdf: singlegpu.py
# 	python3 singlegpu.py results-M\=320.csv $* 4 0

single-gpu-flops.pdf: single-gpu-flops.py
	python3 single-gpu-flops.py results-M=320.csv 8 128

single-gpu-benchmarks.pdf: single-gpu-benchmarks.py results-single-gpu.csv
	python3 single-gpu-benchmarks.py results-single-gpu.csv

weak-scaling-64-4.pdf: weak-scaling.py results-increasingM-weakscaling-P64-N4.csv
	python3 weak-scaling.py results-increasingM-weakscaling-P64-N4.csv true weakscaling-P64-N4.pdf

weak-scaling-128-4.pdf: weak-scaling.py results-increasingM-weakscaling-P128-N4.csv
	python3 weak-scaling.py results-increasingM-weakscaling-P128-N4.csv false weakscaling-P128-N4.pdf

weak-scaling: weak-scaling-64-4.pdf weak-scaling-128-4.pdf

large-8GPUs: max_d_only_speedup.py
	python3 max_d_only_speedup.py 4 64 $@.pdf s results-N\=320-8GPU.csv results-N\=320-4GPU.csv results-N\=320-2GPU.csv results-N\=320-1GPU.csv

# batch_size-8GPUs: increasing_batch_size.py
# 	python3 increasing_batch_size.py $@.pdf s results-increasingN-8GPU.csv results-increasingN-4GPU.csv results-increasingN-2GPU.csv results-increasingN-1GPU.csv

gld_requests: gld_requests.py
	python3 gld_requests.py profile.csv $@.pdf

kernel_selection-small: non_power_two.py
	python3 non_power_two.py results-non-power-two-N=16.csv 4 64 $@.pdf s True

kernel_selection-large: non_power_two.py
	python3 non_power_two.py results-non-power-two-N=320.csv 4 64 $@.pdf s True

clean:
	rm -f *.pdf
